Bayesian Localization and Uncertainty Quantification of Trace Species in Two-Dimensional SIMS Imaging

To enable accurate localization of trace species on material surfaces, we propose a Bayesian framework for analyzing two-dimensional (2D) secondary ion mass spectrometry (SIMS) imaging data. SIMS is widely used in semiconductor manufacturing, materials science, geology, environmental science, and life sciences because of its high sensitivity and excellent elemental and isotopic specificity. However, precise localization remains challenging because of primary ion beam broadening, overlap between neighboring ion distributions, and limited ion counts. The underlying distribution of trace species is modeled as a superposition of two-dimensional Gaussian peaks. To account for the stochastic nature of low-count measurements, the detected ion counts are assumed to follow a Poisson likelihood within a Bayesian framework. Posterior distributions of the peak parameters are estimated using replica-exchange Monte Carlo (REMC), enabling stable inference together with quantitative uncertainty estimation under low-count conditions. The proposed method is first validated using synthetic datasets with known ground truth and is then applied to SIMS measurements of semiconductor samples containing regularly arranged gold (Au) dots with diameters ranging from 0.4 to 2.0~$\mu$m, using scanning electron microscopy (SEM) images as the reference. Optimization of the measurement conditions reduced the relative localization error for 0.4~$\mu$m dots from 5.1$\%$ to 1.9$\%$. These results demonstrate accurate submicrometer localization with statistically rigorous uncertainty quantification in 2D SIMS imaging.

==> sections/2.5_emc_algorithm.tex <==
We employ the exchange REMC algorithm for Bayesian inference, following the framework proposed by Nagata \textit{et al.}\cite{Nagata2012,Nagata2019}.  The REMC algorithm is a Markov chain Monte Carlo (MCMC) algorithm designed to efficiently sample from complex posterior distributions~\cite{Hukushima1996}.

To sample from the posterior distribution $p(\boldsymbol{\Theta}|\mathbf{Y})$ 
defined in Section~\ref{sec:2.4_bayesian}, the REMC method introduces a set of 
replicated distributions parameterized by an inverse temperature $\beta$. The replicated distributions at different inverse temperatures 
are defined as

\begin{equation}
p_{\beta}(\boldsymbol{\Theta}|\mathbf{Y})
\propto
\exp\left(-\beta N E_N(\boldsymbol{\Theta})\right)
p(\boldsymbol{\Theta}),
\end{equation}

where $\beta \in [0,1]$ controls the smoothness of the 
distribution. When $\beta = 1$, the original posterior 
distribution is recovered, while smaller values of $\beta$ 
correspond to flatter distributions that facilitate global exploration 
of the parameter space. In the REMC framework, a set of replicas 
$\{\boldsymbol{\Theta}_m\}_{m=1,...,M}$ is simulated in parallel, 
each associated with a different inverse temperature $\beta_m$ 
such that $0 \leq \beta_1 < \cdots < \beta_M = 1$.
\

The algorithm consists of two types of updates.

\begin{description}

\item[Step 1: Local update]
For each replica, the parameter set $\Theta_m$ is updated using the Metropolis--Hastings algorithm based on the corresponding distribution $p_{\beta_m}(\Theta \mid \mathbf{Y})$. For continuous parameters, adaptive step-size tuning based on the Robbins--Monro process is employed to maintain an appropriate acceptance rate and improve sampling efficiency~\cite{Garthwaite2016,Okajima2021}.

\item[Step 2: Exchange between neighboring replicas]
To enhance sampling efficiency, exchanges of configurations between neighboring replicas are proposed. A swap between replicas $m$ and $m+1$ is accepted with probability

\begin{equation}
p(\Theta_m \leftrightarrow \Theta_{m+1})
=
\min(1,\nu),
\label{eq:swap_prob}
\end{equation}

where

\begin{equation}
\begin{aligned}
\nu
&=
\frac{
p_{\beta_m}(\Theta_{m+1}\mid\mathbf{Y})
\,\,
p_{\beta_{m+1}}(\Theta_m\mid\mathbf{Y})
}{
p_{\beta_m}(\Theta_m\mid\mathbf{Y})
\,\,
p_{\beta_{m+1}}(\Theta_{m+1}\mid\mathbf{Y})
}
\\
&=
\exp
\left[
(\beta_{m+1}-\beta_m)
N
\left(
E_N(\Theta_{m+1})
-
E_N(\Theta_m)
\right)
\right].
\end{aligned}
\label{eq:swap_ratio}
\end{equation}

\end{description}

Through these updates, which combine local Metropolis updates with replica exchanges between different temperatures, REMC efficiently explores the posterior distribution. After discarding the burn-in samples, the parameter samples from the replica with inverse temperature $\beta = 1$ are regarded as samples from the posterior distribution $p(\boldsymbol{\theta} \mid \mathbf{Y})$. The maximum a posteriori (MAP) estimate is then obtained by selecting the sampled parameter set with the smallest value of the negative log-posterior:

\begin{equation}
E(\Theta) = -\log p(\Theta \mid Y)
= E_N(\Theta) - \frac{1}{N} \log p(\Theta),
\end{equation}

where $E_N(\Theta)$ is the empirical energy function defined in Eq.~\eqref{eq:energy}, and $p(\Theta)$ is the prior distribution defined in Eq.~\eqref{eq:prior_total}.

==> sections/2.6_roi.tex <==
In this study, the observed SIMS image is partitioned into regions of interest (ROIs) such that each ROI contains a single localized trace species. Figure 4 shows representative GT Au dots located at different image positions together with their corresponding ROIs. Under this setting, the observed SIMS image in each ROI is represented by a forward model consisting of a single two-dimensional Gaussian component ($K = 1$), and the corresponding model parameters are inferred independently by Bayesian inference.


\begin{figure}[h]
\centering
\includegraphics[width=0.7\columnwidth]{figures/fig1.png}
\caption{
Regions of interest (ROI) segmentation. The observed SIMS image is segmented into ROIs, each containing a single localized signal, and parameter estimation is performed independently for each ROI.
}
\label{fig:roi_schematic}
\end{figure}


